Mobile IMUs Reveal Driver's Identity From Vehicle Turns

As vehicle maneuver data becomes abundant for assisted or autonomous driving, their implication of privacy invasion/leakage has become an increasing concern. In particular, the surface for fingerprinting a driver will expand significantly if the driver's identity can be linked with the data collected from his mobile or wearable devices which are widely deployed worldwide and have increasing sensing capabilities. In line with this trend, this paper investigates a fast emerging driving data source that has driver's privacy implications. We first show that such privacy threats can be materialized via any mobile device with IMUs (e.g., gyroscope and accelerometer). We then present Dri-Fi (Driver Fingerprint), a driving data analytic engine that can fingerprint the driver with vehicle turn(s). Dri-Fi achieves this based on IMUs data taken only during the vehicle's turn(s). Such an approach expands the attack surface significantly compared to existing driver fingerprinting schemes. From this data, Dri-Fi extracts three new features --- acceleration along the end-of-turn axis, its deviation, and the deviation of the yaw rate --- and exploits them to identify the driver. Our extensive evaluation shows that an adversary equipped with Dri-Fi can correctly fingerprint the driver within just one turn with 74.1%, 83.5%, and 90.8% accuracy across 12, 8, and 5 drivers --- typical of an immediate family or close-friends circle --- respectively. Moreover, with measurements on more than one turn, the adversary can achieve up to 95.3%, 95.4%, and 96.6% accuracy across 12, 8, and 5 drivers, respectively.

==> body/background__Cho_Kyong_Tak___________________________________________________2017-05-02_.tex <==
\section{Background}
\label{sec:backgroud}

\subsection{Related works}
% TODO: Highlight three constraints: 1. Using CAN; 2. Needs long and fixed route; 3. Use the label of training data set as given

==> body/introduction_original.tex <==
%%%% Following is the original introduction %%%%
{\color{magenta} --------- Following is the original introduction ---------}
\section{Introduction}\label{sec:intro}
Everyone drives differently --- everyone should have experienced that depending on who the driver is, the ride comfort/discomfort or the impression of riding can be quite different. On one hand, the fact that different drivers have different habits/tendencies in maneuvering the vehicle (e.g., left/right turn, lane changes, acceleration/deceleration) has led researchers and vehicle manufacturers to build systems which can identify/fingerprint the driver solely based on sensor data (without oversight) and use the information for various personalized driver-assistance applications. For example, depending on who the (detected) driver is, the vehicle adjusts its settings to fit the driver's preferences such as the driver seat, temperature, radio station, mirror placement, etc.~\cite{single_turn2016}. Another example is using the information for anti-theft purposes~\cite{knowmaster}. On the other hand, the feasibility of such a {\em driver identification/fingerprinting} has led to a controversial and undesirable consequence: privacy breach/violation. The authors of \cite{yoshi2016} showed how an adversary with access to in-vehicle data can determine who the driver is, i.e., fingerprint the driver (without oversight), and thus abuse that information. That is, any driver fingerprinting scheme can lead to privacy violation, thus becoming a double-edged sword.

While existing driver fingerprinting  schemes~\cite{yoshi2016,knowmaster,single_turn2016} 
can be a serious privacy threat when used by an adversary, their practicability 
to adversaries remains limited due to their requirements: 1) control of a compromised dongle plugged
in the vehicle's On-Board Diagnostic (OBD-II) port or a compromised Electronic Control Unit (ECU) 
on the in-vehicle network;
2) the capability of those compromised components to read in-car data; and
3) knowledge of which in-car messages contain which sensor data
(e.g., break pedal position, steering wheel angle) and how those raw 
data values can be translated to the actual sensor values~\cite{yoshi2016}. 
Note that how sensor data is encoded is different per 
vehicle manufacturer and even per vehicle model-year~\cite{busoff}.
Considering the fact that reading in-car sensor data via the OBD-II port is 
becoming more and more difficult (or even impossible), especially due to 
restrictions imposed by the vehicle manufacturers~\cite{obdblock}, one might 
argue that the adversary may not even be able to satisfy the first two requirements. 
Even with access, some might also argue that in order to know which 
in-car messages contain the required sensor data for driver identification, the adversary may 
be required to reverse-engineer messages, which is quite painstaking and often incomplete~\cite{busoff, cids}. 
Thus, this approach is not very practical for an adversary (with such restrictions 
and hurdles) to identify/fingerprint the driver. 

To overcome this impracticality, we explore whether an adversary can identify the driver 
even with much less effort and resources, i.e., {\em without} meeting the above-mentioned requirements.
Specifically, we propose a drastically different scheme, called \name\ 
(\underline{Dri}ver \underline{Fi}ngerprint), which can 
correctly identify/fingerprint the driver even when he only has access to a 
mobile IMU (Inertial Measurement Unit), which we refer to as an electronic
component comprised of the gyroscope, accelerometer, and (sometimes) the 
magnetometer, such as IMU sensors on commodity smartphones.
Since this is the only requirement for \name\ to achieve driver 
fingerprinting, an adversary exploiting it can easily breach the driver's privacy as follows:
\begin{enumerate}
\item {\bf Any device with an IMU:} Since IMUs are available in (i) all commodity
smartphones, which drivers are very likely to carry while driving, (ii) wearable devices, 
some COTS (Commercial-Off-The-Shelf) devices, and (iii) even in OBD-II dongles 
(either purchased from a third-party or received from an 
auto-insurance company)~\cite{woot_tele}, the adversary can fingerprint the 
driver using {\em any} of these devices, i.e., no restriction on which device to use.
\item {\bf Zero-permission:} Since IMU sensors can be accessed without requiring
user permission or oversight, i.e., zero-permission mobile sensors, an 
adversary exploiting \name\ can easily and stealthily fingerprint the driver. 
In contrast to existing approaches, this also implies that the adversary does 
\textit{not} require to have permission of accessing in-car data or knowledge 
on how to decode/translate it. Hence, from the attacker's point of view, driver 
fingerprinting becomes much more practical and simpler with \name.
\end{enumerate}

Albeit IMU being the only available resource, \name\ achieves 
driver fingerprinting via its new unique approach. By reading and utilizing 
the gyroscope and accelerometer sensor readings, \name\ first detects the event 
of a {\em left/right turn}. A turn is detected 
by accumulating the yaw rate measured by the gyroscope. When the driver 
makes a left turn, the accumulated value would approximately be -90$^{\circ}$ 
whereas for a right turn it would be 90$^{\circ}$. The reason why \name\ 
focuses on only turns for fingerprinting is that these events are the 
ones which reflect the unique behavior of the driver and most importantly are 
less likely to be affected by traffic conditions than other maneuvers. 
For example, deceleration can be affected greatly by the car in front whereas 
left/right turn is not. 
%Meanwhile, we will later discuss the possible 
%impacts/interruptions from pedestrians.

Once \name\ detects a turn, it derives three new proposed features:
1) the acceleration along the end-of-turn axis, which is defined
	as the axis orthogonal to the vehicle's direction when the turn started, 
2) the deviation in the first feature, and
3) the deviation in the yaw rate.
These features function as the core of \name's driver fingerprinting as they 
reflect the driver's unique behavior --- they are only affected by how the 
driver actually turns the steering wheel or how s/he presses the 
acceleration/brake pedal while making the turn, i.e., they are dependent on 
only the driver's actions. 
Through extensive experimental evaluations, we will later show that these 
features vary with drivers, but {\em not} with cars or routes. 
Once these three features are derived for the detected turn, \name\ derives various percentiles and 
their autocorrelations which are then used to construct the feature vector for 
machine classifiers, such as Random Forest, Naive Bayes, and SVM.  
\name\ can, therefore, fingerprint the driver with a high probability, even when s/he makes just one left/right turn. 
As more turns are made by the driver within a trip, \name\ exploits such accumulated information 
for driver fingerprinting to reduce possible false positives/negatives, thus enhancing its accuracy.
In addition to the driver fingerprinting, we also discuss how an adversary may
utilize its IMU measurements to construct a well-formulated training dataset 
from scratch, which is essential for the underlying machine classifiers. 
Note that all existing studies (had to) assume that the training dataset, which 
has the correct labels, was {\em given} to the adversary, which does not hold 
in practice.

We have evaluated \name\ extensively by collecting IMU sensor data from a 
smartphone while 12 different drivers (9 males, 3 females) were driving either 
around the campus or in an urban/rural area. 
%Using the recordings as a database, we used 
%the classifiers with 10-fold cross validation
%to investigate whether \name\ can correctly identify/fingerprint the driver.
Our results have shown that by using \name, the driver can be  
fingerprinted/identified within one left/right turn, with 74.1\% accuracy 
across 12 drivers, 83.5\% across 8 drivers, and 90.8\% across 5 drivers. 
Such a result is significant in that \name\ achieves high accuracy {\em with just one turn},
which is in sharp contrast to existing studies that require several minutes of measurements 
from tens of in-car sensors. More importantly, \name\ achieved it with only two zero-permission 
mobile IMU sensors: gyroscope and accelerometer.
Moreover, as the driver made 8 (either left or right) turns, \name\ 
was able to achieve a fingerprinting accuracy of 95.3\%, 95.4\%, and 96.6\% 
across the 12, 8, and 5 drivers, respectively.

For an adversary exploiting \name, since s/he can identify the driver with only 
an IMU (readily accessible on a smartphone, off-the-shelf device, or a 
plugged-in OBD-II dongle), many more scenarios exist in 
which the driver's privacy can be breached, compared to those considered 
possible before (when using in-car data). We detail such new scenarios when 
discussing the threat model in Section~\ref{sec:threatModel}.

This paper makes the following main contributions:
\begin{itemize}
\item[1.] Discovery of three new features which are shown to
	be distinct between different drivers and independent of vehicles and trip routes;
\item[2.] Development of a novel scheme, \name, which extracts the new 
	features when the driver is making a left/right turn and thus achieves 
	driver fingerprinting (as soon as the driver makes the turn) with a high 
	accuracy; and
\item[3.] Implementation and extensive evaluation of \name\ using a commodity 
smartphone.
\end{itemize}

The rest of this paper is organized as follows. 
The next section introduces the related work of driver fingerprinting while
Section 3 details the threat model under consideration and states our research goal.
Sections 4 and 5 details and evaluates \name, respectively.
Section 6 discusses the various aspects of \name.
Finally, we conclude in Section 7.

==> body/threatModel_original.tex <==
%%%%%%%%

{\color{magenta} --------- Following is the original Problem Statement --------}
\subsection{Adversary Model}
In order to identify/fingerprint the driver via sensor data (reflecting vehicle/driver maneuvering), 
an adversary can collect data from in-car sensors or mobile IMU sensors.
Hence, depending on the adversary's capability and resources, which decide in which way 
he will collect data, we consider two different types of adversaries: {\em high-resource} 
and {\em low-resource} adversaries.

{\bf High-resource adversary.} 
An adversary with access to data of several sensors (e.g., break pedal 
position, steering wheel angle, throttle position) on an in-vehicle network, 
such as Controller Area Network (CAN), is shown to be able to fingerprint the 
driver \cite{yoshi2016, single_turn2016, driver_inertial_sensor, driverID_gmm2007, knowmaster}. 
Despite the rich and low-noise in-car data for the adversary to achieve driver 
fingerprinting, s/he must meet the following minimum requirements (which all 
existing studies assume to have been met).

First, to read and extract sensor values from the in-vehicle network, the adversary 
requires to have access to the sensor. To gain such an access, s/he may either have to
1) remotely compromise an ECU, or 2) have a compromised 
OBD-II dongle plugged in the victim's vehicle in order to read
in-car data.\footnote{Note that drivers try to lower their auto-insurance rates 
by plugging in OBD-II dongles provided by auto-insurance companies or try to 
constantly diagnose their cars using them.}
For the first case, however, depending on the ECU which the adversary 
compromised, s/he may not be able to read {\em all} sensor values of 
interest, mainly because the ECUs which produce those values may reside 
in different in-vehicle networks (e.g., some on high-speed CAN and others on low-speed CAN).
For the second case, even though the adversary has control of a plugged-in and
compromised OBD-II dongle, which, in contrast to a compromised ECU, is 
likely to have access to all sensor values of interest 
(as shown in~\cite{yoshi2016,knowmaster}), if data access from the 
OBD-II port is blocked by the vehicle manufacturer, then the adversary would 
not even be able to access any of in-car data. For security reasons, vehicle manufacturers 
are increasingly blocking/prohibiting access to in-car data through the OBD-II port 
except when the vehicle is stable~\cite{obdblock}.

Even when the adversary has gained access to in-vehicle network messages,  
the adversary must still meet the second requirement: (i) understanding
where and in which message the sensor value (of interest) is contained, and (ii) knowing 
how to translate them into actual sensor values (e.g., transformation 
coefficients for addition/multiplication of raw sensor data~\cite{yoshi2016}). 
In-vehicle network messages are encoded by the vehicle 
manufacturers and the ``decoding book'', which allows one to translate the raw 
data is proprietary to them. Therefore, unless the adversary has 
access to such a translator, s/he would have to reverse-engineer the messages, 
which could be quite painstaking and also often incomplete.

Although the adversary may have abundant resources to fingerprint
the driver, meeting these two requirements may be difficult or even impossible.
Despite such restrictions/hurdles, we refer to an adversary which {\em does 
have} the capability and resources to meet all these conditions as a {\em 
high-resource adversary}.

{\bf Low-resource adversary.}
Instead of fingerprinting the driver using in-car data, an adversary 
can attempt to exploit the readings from mobile IMU sensors, 
possibly due to lack of his/her 
technical expertise on in-car data or given resources.
Compared to in-car sensors, mobile IMU sensors can only provide limited 
information. For example, in-car CAN data from a vehicle may 
include tens of different sensor values, including the brake/acceleration 
pedal position, engine torque, requested torque, engine RPM, etc. Whereas, 
mobile IMU sensor data streams would only have 3 different types of data, which 
are gyroscope, accelerometer, and magnetometer data. Given such a limited 
number of distinct data, we consider such an adversary as a {\em 
low-resource adversary}. 

\kt{Although his resources might be limited, since IMU sensors are readily and 
vastly available, a low-resource adversary would have a much {\em larger} 
attack surface than that open to a high-resource adversary.}
%in all smartphones, wearable devices, some off-the-shelf devices, 
%and even in OBD-II dongles~\cite{woot_tele}, 
More importantly, as access to those sensors does not require user permission 
or oversight (i.e., zero-permission sensors), the technical barrier for a
low-resource adversary would be much lower than that for a high-resource attacker.

When the low-resource adversary exploits the victim's mobile devices (e.g., smartphones, wearables) 
for collecting IMU sensor data, their unique identifiers are not given to him
for free, i.e., not zero-permission. 
Android requires the user's permission if an app wants to read unique 
identifiers such as IMEI (International Mobile Equipment Identifier) and IMSI 
(Subscriber Identifier)~\cite{android_permission,accel_NDSS2014}. For privacy 
protection, Apple is preventing apps from reading them~\cite{apple_tracking}.
Although there are ways to identify the device (or its owner) with 
zero-permission (e.g., via accelerometer fingerprints~\cite{accel_NDSS2014}), 
they do not necessarily tell who the driver of a vehicle is.

\subsection{Motivating Scenarios}
\label{subsec:motivating_cases}
Several example scenarios in which a high-resource adversary ---
who has access to in-vehicle data through a plugged-in OBD-II dongle ---
can violate the driver's privacy were discussed in \cite{yoshi2016}.
One example was an insurance company, which knows who the driver is via
its supplied OBD-II dongle, may cancel one's insurance if some other person not
under the coverage drives the vehicle. Another was the OBD-II dongle back-end
service sending text messages with targeted ads based on who the driver is. 
However, since relatively little is known about what a low-resource adversary 
can (similarly or even better) do with his limited resources, we present 
several new example scenarios in which he may maliciously exploit his mobile 
IMU sensor data against the driver's will and thus exacerbate the potential 
damages.
%Since our goal, however, is to understand what a low-resource adversary can 
%(similarly or even better) do with his limited resources, we present several 
%new example scenarios in which he may maliciously exploit his mobile IMU 
%sensor 
%data against the driver's will and thus exacerbate the potential damages.
\begin{itemize}
\item {\bf {Driver distraction.}}
Distracted driving caused by use of mobile devices creates serious risks for injuries and even deaths on roads \cite{distracted_driving}. 
Therefore, Mallory who is aware of such a risk can effectively endanger Alice by mounting a Telephone Denial-of-Service (TDoS) 
attack on her smartphone (e.g., phone bombing) \cite{tdos_report}, thus incurring a high level of distraction.
Note that this attack only requires Mallory to accurately detect that Alice is 
indeed the driver --- as she might be just a passenger, in which case 
distraction cannot effectively endanger the victim. 
To this end, if Alice's mobile device (e.g.,  Alice's smartphone with a compromised app controlled by Mallory) transmits 
the IMU sensor data to Mallory, he can analyze the IMU data to verify the driver's identity.
%Distracted driving caused by use of mobile devices creates enormous potential for injuries and even deaths on roads \cite{distracted_driving}. Suppose Mallory who is aware of such a fact can effectively endanger Alice by mounting a telephone denial-of-service (TDoS) attack on her smartphone (e.g., phone bombing) \cite{tdos_report} and thus incur a high level of distraction.
%Also suppose that Mallory has his (compromised) app installed on Alice's phone.
%Since the attack requires Mallory to accurately detect that Alice is indeed the driver --- as she might be just a passenger --- Mallory reads the IMU sensors to verify it.
	
\item {\bf {Precision-guided vehicle attack.}}
Suppose Mallory attached a malicious device on the exterior (e.g., underneath the body) of Alice's vehicle while it was parked. 
Examples of such a malicious device can either be hardware which spoofs
the wheel speed sensors and thus activates the Anti-Brake System (ABS)~\cite{ABSattack}, 
or hardware which jams or spoofs the tire pressure sensor of the vehicle~\cite{tpms}.
If Mallory wants to activate his device {\em only when} he is certain that 
Alice is actually on board, then the best possible case would be when 
Alice is actually driving the car. Note that Alice's car could be driven
by someone else. In such a case, if Mallory's device has IMU sensors built in,
then he can exploit them to verify that Alice is driving. 
%(with no need to read in-car data). 
Also, Mallory may exploit IMU sensors on Alice's phone.

\item {\bf {Locating a specific driver.}}
Suppose Alice and her husband Bob share the same vehicle. 
Also suppose Mallory has control of a malicious smartphone application, which has permission 
only to read the GPS data, installed on both Alice's and Bob's phones.
Using that app, Mallory wants to know on what road "Alice" is currently driving. 
The only situation in which Mallory would be {\em certain} about this is when Alice is the driver, 
since the car might be driven by Bob as well.
Hence, Mallory exploits the app to further read the "zero-permission"
IMU sensors to determine whether Alice is driving, and the GPS data
to determine on which road Alice is driving. 
Even when Mallory does not have access to the GPS data, he may infer Alice's 
location using zero-permission mobile IMUs as in \cite{inferroute}.
If Alice and Bob are both on the vehicle, note that Mallory can identify the 
driver using either of their smartphones.
%If Mallory also has access to a navigation app's waypoint data 
%(e.g., a destination set in Google Map), then he would even be certain of 
%where Alice is heading to.

\item {\bf {Possible information abuse.}}
Suppose a ride-sharing company (or its mobile application) called 
{\em RideShare} wants only the authorized drivers to drive the registered 
vehicle. However, the vehicle owner decides to let someone else drive the 
vehicle, instead. In such a case, {\em RideShare} may abandon the rights of the 
vehicle owner to register and drive for it.
\end{itemize}

\subsection{Research Goal}\label{sec:problem}
Researchers have already demonstrated the feasibility of a high-resource 
adversary (with access to in-car data) breaching the driver's privacy by 
fingerprinting/identifying him/her
\cite{yoshi2016, single_turn2016, driver_inertial_sensor, driverID_gmm2007, knowmaster}.
Hence, we will focus on what a low-resource adversary can achieve, and 
aim to shed light on the unexplored issue of:

\vspace{0.3em}
\emph{``How will a low-resource adversary be as capable as a
	high-resource adversary in fingerprinting the driver, albeit his limited 
	resources, i.e., having access to only mobile IMUs?"}
\vspace{0.3em}

%Our answer to this question is: if such a low-resource adversary exploits  
%\name\ (to be elaborated in Section~\ref{sec:system}), it is indeed
%possible for him to fingerprint the driver as the high-resource adversary can; 
%sometimes even better than the high-resource adversary within just one vehicle 
%turn.
It is important to note that the example scenarios discussed in 
Section~\ref{subsec:motivating_cases}, ironically, can only be 
achieved by a low-resource adversary (capable of driver fingerprinting), 
but not by the high-resource adversary, since these are based on utilizing the 
mobile IMU sensors either on smartphones, wearable devices, or on off-the-shelf 
devices, and do not require in-car data access.
Moreover, even under scenarios in which a high-resource adversary 
utilizes a compromised OBD-II dongle to identify the driver, the low-resource
adversary can {\em also} achieve it, mainly because those OBD-II 
dongles also have mobile IMU sensors~\cite{woot_tele}. 
This leads to an important but critical conclusion that the low-resource 
adversary will in fact breach/violate privacy of the driver in more 
scenarios than the high-resource adversary, even subsuming all those mentioned 
in \cite{yoshi2016} (where the high-resource adversary exploited OBD-II 
dongles).

